CreativeBench: Benchmarking and Enhancing Machine Creativity via Self-Evolving Challenges

The saturation of high-quality pre-training data has shifted research focus toward evolutionary systems capable of continuously generating novel artifacts, leading to the success of AlphaEvolve. However, the progress of such systems is hindered by the lack of rigorous, quantitative evaluation. To tackle this challenge, we introduce CreativeBench, a benchmark for evaluating machine creativity in code generation, grounded in a classical cognitive framework. Comprising two subsets -- CreativeBench-Combo and CreativeBench-Explore -- the benchmark targets combinatorial and exploratory creativity through an automated pipeline utilizing reverse engineering and self-play. By leveraging executable code, CreativeBench objectively distinguishes creativity from hallucination via a unified metric defined as the product of quality and novelty. Our analysis of state-of-the-art models reveals distinct behaviors: (1) scaling significantly improves combinatorial creativity but yields diminishing returns for exploration; (2) larger models exhibit ``convergence-by-scaling,'' becoming more correct but less divergent; and (3) reasoning capabilities primarily benefit constrained exploration rather than combination. Finally, we propose EvoRePE, a plug-and-play inference-time steering strategy that internalizes evolutionary search patterns to consistently enhance machine creativity.

==> tables/Reverse-engineering.tex <==
\begin{algorithm}[t]
\caption{Construction Pipeline for CreativeBench-Combo}
\label{alg:combo_pipeline}
\begin{algorithmic}[1]
\Require Seed code components $\mathcal{D}$, Foundation Model $\mathcal{M}$, Sandbox $\mathcal{E}$
\Ensure Combinatorial Dataset $\mathcal{S}_{combo}$
\State $\mathcal{S}_{combo} \leftarrow \emptyset$
\For{each iteration $i = 1$ to $N$}
    \State \textcolor{gray}{\emph{// Step 1: Solution Fusion}}
    \State $S_{ref} \leftarrow \mathcal{M}.\text{fuse\_components}(\mathcal{D})$ 
    \If{$\mathcal{E}.\text{execute}(S_{ref}) \neq \text{Success}$} 
        \State \textbf{continue}
    \EndIf
    
    \State \textcolor{gray}{\emph{// Step 2: Test Function Generation}}
    \State $I \leftarrow \mathcal{M}.\text{generate\_inputs}(S_{ref})$
    \State $O \leftarrow \mathcal{E}.\text{get\_outputs}(S_{ref}, I)$ \Comment{Get ground truth via sandbox}
    \State $T_{func} \leftarrow \text{construct\_test\_function}(I, O)$
    
    \State \textcolor{gray}{\emph{// Step 3: Problem Synthesis (Reverse Engineering)}}
    \State $P_{desc} \leftarrow \mathcal{M}.\text{synthesize\_problem}(S_{ref}, T_{func})$
    
    \State \textcolor{gray}{\emph{// Step 4: Filtering}}
    \If{$\text{Filter}(P_{desc}, T_{func})$ is \textbf{True}}
        \State $\mathcal{S}_{combo} \leftarrow \mathcal{S}_{combo} \cup \{(P_{desc}, S_{ref}, T_{func})\}$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

==> tables/Self-play.tex <==
\begin{algorithm}[t]
\caption{Construction Pipeline for CreativeBench-Explore}
\label{alg:explore_pipeline}
\begin{algorithmic}[1]
\Require Seed Task $T_{seed} = (P, S_{base})$, Generator $\mathcal{G}$, Solver $\mathcal{M}$, Sandbox $\mathcal{E}$, Judge $\mathcal{J}$
\Ensure Exploratory Dataset $\mathcal{S}_{explore}$
\State $\mathcal{S}_{explore} \leftarrow \emptyset$
\For{each task $(P, S_{base}) \in T_{seed}$}
    \State \textcolor{gray}{\emph{// Step 1: Targeted Constraint Injection}}
    \State $\mathcal{C} \leftarrow \mathcal{G}.\text{analyze\_and\_constrain}(S_{base})$ \Comment{E.g., forbid sort(), max()}
    
    \State \textcolor{gray}{\emph{// Step 2: Reference-Guided Refinement (Self-Play)}}
    \State $S_{curr} \leftarrow S_{base}$
    \State $Solved \leftarrow \textbf{False}$
    
    \While{\textbf{not} $Solved$ \textbf{and} steps $<$ MaxSteps}
        \State $S_{new} \leftarrow \mathcal{M}.\text{refine}(S_{curr}, \mathcal{C}, \text{Feedback})$
        
        \State $v_{exec} \leftarrow \mathcal{E}.\text{execute}(S_{new})$ \Comment{Check correctness}
        \State $v_{const} \leftarrow \mathcal{J}.\text{check\_constraint}(S_{new}, \mathcal{C})$ \Comment{Check novelty}
        
        \If{$v_{exec} \land v_{const}$}
            \State $\mathcal{S}_{explore} \leftarrow \mathcal{S}_{explore} \cup \{(P, \mathcal{C}, S_{new})\}$
            \State $Solved \leftarrow \textbf{True}$
        \Else
            \State $\text{Feedback} \leftarrow \text{generate\_feedback}(v_{exec}, v_{const})$
            \State $S_{curr} \leftarrow S_{new}$
        \EndIf
    \EndWhile
\EndFor
\end{algorithmic}
\end{algorithm}

==> tables/base_model.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.15}
\resizebox{0.88\textwidth}{!}{
\begin{tabular}{l | c c c | c c c}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{CreativeBench-Explore}} &
\multicolumn{3}{c}{\textbf{CreativeBench-Combo}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \textbf{Pass Rate} & \textbf{Novelty} & \textbf{Creativity}
& \textbf{Pass Rate} & \textbf{Novelty} & \textbf{Creativity} \\
\midrule

qwen2.5-72b-instruct &
0.172131 & 0.078975 & 0.012305 &
0.268349 & 0.547830 & 0.152472 \\

deepseek-v3-0324 &
0.213115 & 0.070390 & 0.012045 &
0.412844 & 0.546044 & 0.227645 \\

claude-3-5-sonnet-20240620 &
0.338798 & 0.083785 & 0.025579 &
0.425076 & 0.500354 & 0.214648 \\

gemini-2.5-flash-lite &
0.234973 & 0.131359 & 0.027314 &
0.363914 & 0.549348 & 0.201012 \\

gemini-2.5-pro &
0.538251 & 0.193790 & 0.106915 &
0.441896 & 0.535227 & 0.238673 \\

\bottomrule
\end{tabular}
}
\caption{Combined performance of major LLMs on CreativeBench, reporting averaged Pass Rate, Novelty, and Creativity for both Explore and Combo settings.}
\label{tab:combined_creativebench_no_alias}
\end{table*}

